Modelling the early mass-ejection in jet driven protostellar outflows. Lessons from Cep E

We have used the axisymmetric chemo-hydrodynamical code WALKIMYA-2D to numerically model and reproduce the physical and CO emission properties of the jet-driven outflow from the intermediate-mass protostar Cep E, which was observed at $\sim 800$au resolution in the CO $J=2\to 1$ line with the IRAM interferometer. Our simulations take into account the observational constraints available on the physical structure of the protostellar envelope to provide constraints on the dynamics of the inner protostellar environment from the study of the outflow/jet propagation away from the launch region. WALKIMYA-2D successfully reproduces the main qualitative and quantitative features of the Cep E outflow and the jet kinematics, naturally accounting for their time variability. Signatures of internal shocks are detected as knots along the jet. In the early times of the ejection process, the young emitted knots interact with the dense circumstellar envelope through high-velocity, dissociative shocks, which strongly decrease the CO gas abundance in the jet. As time proceeds, the knots propagate more smoothly through the envelope and dissociative shocks disappear after $\sim 10^3$ yr. The distribution of CO abundance along the jet shows that the latter bears memory of the early dissociative phase in the course of its propagation. Analysis of the velocity field shows that the jet material mainly consists of gas entrained from the circumstellar envelope and accelerated away from the protostar at $700$ au scale. As a result, the overall jet mass loss rate appears higher than the actual mass ejection rate by a factor $\sim 3$. Numerical modeling of the Cep E jet-driven outflow and comparison with the CO observations have allowed us to peer into the outflow formation mechanism with unprecedented detail and to retrieve the history of the mass-loss events that have shaped the outflow.

==> sec4_others.tex <==
\section{Other models }
\label{sec:other}

The first difference between M4 and the other models is that the main cavity in the density map is less turbulent than in the previous models, but the width remains almost constant for most of the outflow length, in agreement with the Cep\,E observations.   

\begin{table}[]
    \centering
    \begin{tabular}{l|c|c|c|c|c|c} \hline\hline
Parameter    & M1 & M2 & M3& M4& \multicolumn{2}{c}{Cep\,E} \\
             &    &    &   &  & \multicolumn{2}{c}{North South} \\
    \hline
$M_{j}\, [10^{-2}$M$_\odot]$ & 5  & 0.75& 1.5 & 2.25 & 2.0 & 6.0\\
$M_{o}[$M$_\odot]$           & 2.9& 1.3 & 1.2 & 2.3  & 2.0 &  2.0\\
$z_{bs}[\,10^3$au$]$         & 41  & 31 & 38  & 37   & 30. & \\
$r_{max}[\,10^3$au$]$        &5.3  & 1.5 &3.6 & 3.7  & 4. & \\
        \hline
%        $v_t$ & & &     
    \end{tabular}
    \caption{
Outflow physical properties derived from CO emissivity maps at 1500~yr in the four numerical simulations (M1-- M4) and comparison with the Cep\,E observational values: jet mass $M_j$, outflow mass $M_{o}$, jet length $z_{bs}$, maximum jet radius $r_{max}$. These values are taken from \citet{Lefloch2015} and \citet{Ospina-Zamudio2019} and have been corrected for the revised distance to the source.  }
    \label{tab:results}
\end{table}

%\begin{table}[]
%    \centering
%    \begin{tabular}{l|c|c|c|c|c} \hline\hline
%    Parameter    & M1 & M2 & M3& M4& Cep\,E\\
%    \hline
%        $M_{j}\, [10^{-2}$M$_\odot]$ & 5 & 0.75 & 1.5 & 2.25 & 2.0\\
%        $M_{o}[$M$_\odot]$ & 2.9  & 1.3 & 1.2  & 2.3&2 \\
%        $z_{bs}[\,10^3$au$]$ & 41  & 31 & 38 & 37& 30\\
%        $r_{max}[\,10^3$au$]$  &5.3  & 1.5 & 3.6  & 3.7& 4\\
%        \hline
%%        $v_t$ & & &     
%    \end{tabular} 
%    \caption{Outflow physical properties derived from CO emissivity %maps at 1500~yr in the four numerical simulations (M1-- M4) and %comparison with the Cep\,E observational values: jet mass $M_j$, %outflow mass $M_{\odot}$, $z_{bs}$, maximum jet radius $r_{max}$. }
%    \label{tab:results}
%\end{table}
%

%{\bf The ultimate goal of this study is to obtain a fully %coherent modeling of the Cep\,E molecular outflow in agreement %with the observational constraints. In particular,  this work %aims to understand the dynamics of the jet/envelope interaction %near the source and to test the scenario proposed by %\citet{Schutzer2022} for the formation of a molecular gas layer %around the high-velocity jet. }


The four models presented in Table \ref{tab:models} display variations in the ejection radius, the velocity of the injected material, the amplitude of the velocity variation, and the temperature of the injected material. From comparison between the different simulations, we aim to investigate the impact of these parameters on the outflow formation.

To start this comparations we comment on the common results from the simulation grid.  In Figure \ref{fig:jet2000} we show an animation from model M1 numeric density maps from $t=0$ to $2000$ yr. Turning on the jet creates an outflow with a high velocity component and a cocoon that expands laterally creating a “cavity" component at low velocity. Also, the models show a leading jet head
and a series of traveling “internal working surfaces”
(IWS) which are formed as a result of the ejection
time-variability since the slower material interacts with the faster material ejected at later times.  This is an expected result, Raga et al., (1990) and subsequent publications have analyzed the internal shock dynamics. The first working surface must interact with a very dense envelope which makes it decelerate, causing that the second peak in velocity catches up with the first bowshock. 

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[angle=270,width=0.9\textwidth]{figures/jetCepE_ra080.pdf}
%     \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%     \label{fig:jet2000}
% \end{figure*}

%\begin{figure*}[!ht]
%    \centering
%    \includegraphics[angle=0,width=0.9\textwidth]{figures/jetages.pdf}
%    \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%    \label{fig:jet2000}
%\end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[angle=0,width=0.9\textwidth]{figures/t0.pdf}
%     \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%     \label{fig:jet2000}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[angle=0,width=0.9\textwidth]{figures/t500.pdf}
%     \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%     \label{fig:jet2000}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[angle=0,width=0.9\textwidth]{figures/t1000.pdf}
%     \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%     \label{fig:jet2000}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[angle=0,width=0.9\textwidth]{figures/t1500.pdf}
%     \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%     \label{fig:jet2000}
% \end{figure*}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[angle=0,width=0.9\textwidth]{figures/t2000.pdf}
%     \caption{Simulation 2000 yr. Use snapshots for 0,500, 1000, 1500, and 2000 yr}
%     \label{fig:jet2000}
% \end{figure*}


%In order to compare our numerical simulation with CO observations, the emissivity %has been obtained directly from the hydrodynamic simulations assuming LTE. We have %constructed an integrated synthetic CO J=2$\to$ 1 map, for the cavity, with %velocities between 3 to 7~km~s$^{-1}$, and the jet material, with velocities %between 50 to 150~km~s$^{-1}$, convolving the numerical emission with the %corresponding beam size at 830~kpc. 

The integrated synthetic CO map for Model A at 1400 yr  show that the outflow is fragmented along the jet propagation axis. The high velocity component, with knots that also are emission peaks, has a width around 10$^3$~au. Also, the terminal bowshock has no CO emission. It is worth pointing out that the northern jet of Cepheus E is behind the terminal bowshock defined by HH377. This could be explained by CO destruction.
 
 \begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/components-080.jpeg}
    \caption{Logarithmic CO $J=2\to1$ integrated emissivity contour maps of the cavity (Black contours, 3 to 7 km s$^{-1}$) and jet (Blue contours, 50 to 150 km s$^{-1}$) components obtained from the Model A convolving accordingly to the beam size at a distance of 830 kpc at 1400 yr with $r_j=50$~au.(Gray Disk). The frontal shock is represented with the red point {\bf (Use a figure for 2000 yr)}}
    \label{fig:components}
\end{figure}
 

In models M1 to M3, the PV diagram has clearly 2 components at low velocity, corresponding to the cavity, and at high velocity, corresponding to the jet. 

\subsection{Jet radius}

In model M1, we consider a jet with initial jet radius of 100~au, hence twice as large as that of the other models. The jet is  ejected at a mean velocity of $200\kms$. It is therefore the model with the highest  mass injection rate per unit time into the environment (Eq.~\ref{eq:mdot})  $\sim 7.3\times 10^{-6}$. 
The injected material interacts with the dense central core, accelerating it and increasing the amount of gas that is detected at high velocity. 
{\bf It is therefore not surprising that at a similar jet length in both simulations M1 and M4, the outflow is actually wider than in M1.}
According to the simulation, it appears that at $t$= $1500\yr$, when the outflow length is similar to that of Cep\,E, the jet mass amounts to $6\times 10^{-2}$~M$_\odot$, almost six times the injected mass of the jet. {\BF We conclude that ambient material entrainment is still efficient. } 

\begin{figure}[!ht]
     \centering
     \begin{subfigure}
     \includegraphics[width=0.49\textwidth]{figures/M1n}
    \end{subfigure}
    \begin{subfigure}
 \includegraphics[width=0.49\textwidth]{figures/M1pv}
    \end{subfigure}
     \caption{Model M1. Outflowing gas distribution and kinematics at $t$= $1400\yr$. (top)~density field. (bottom)~Position-velocity diagram along the jet main axis.}
     \label{fig:jet1300}
 \end{figure}


% According to the total velocity of the north lobe of Cep E, the outflow should be expanding at 165 km s$^{-1}$. Then, this is a lower limit for the injection velocity, which is not enough to decrease the jet mass in a factor 3, which should be compensated by decreasing also the injection radius. This is explored on Model M2 where we have taken the lower velocity limit and an injection radius of 50 au. However, our simulations show that the effective velocity of the outflow is decelerated from the injection velocity due to the interaction of the jet with the dense central envelope. In this case, the CO J=2$\to 1$ PV diagram in Fig 8b show that the mean terminal velocity is close to be constant around 50 km s$^{-1}$, which is very low compared with the observations. In any case, this PVD shows two very definite components. A low velocity component, associated with the cavity and a high velocity component, that shows a periodical behavior, reflecting the variability in the injection and the internal shocks, where the fast material catches up with the slower material. The velocity gradient, according to the diagram, is around 15 km s$^{-1}$. This is observed in other molecular jets, e.g. Santiago-Garcia et al., (2009). This "jet" component also has a decreasing intensity along the outflow length getting fainter in older shocks.

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M2n}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M2pv}
%   \caption{Position velocity diagram for model Model M2 for the CO J$=2\to1$. There is a low velocity component near the source that is originated from the outflow cavity and a high velocity component coming from the jet.}
%     \label{fig:M2}
% \end{figure}


% Then, in Model M3 we decided to use again an injection velocity of 200 km s$^{-1}$ keeping the injection radius at 50 au, but exploring the amplitude of the relative velocity variability, decreasing it from $8\%$ to $5\%$. This relative amplitude is offtently assumed and can be constrained through simulations. Even when the density map shows a similar structure to the previous models, that is, the length and the width are consistent with the observations, the PV diagram has a high velocity component that exhibits a steep gradient, suggesting that the jet itself is structured in velocity. Again, the intensity decreases along the jet. The mean velocity is also less than expected, but the structure, length, and width remain very similar to the observed ones.

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M3n}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M3pv}
%     \caption{Position velocity diagram for model M3 for the CO J$=2\to1$. There is a low velocity component near the source that is originated from the outflow cavity and a high velocity component coming from the jet.}
%     \label{fig:M3}
% \end{figure}


\subsection{Jet velocity} 
According to the total velocity of the north lobe of Cep E, the outflow should be expanding at 165 km s$^{-1}$. Then, this is a lower limit for the injection velocity, which is not enough to decrease the jet mass in a factor 3, which should be compensated by decreasing also the injection radius. This is explored on Model M2 where we have taken the lower velocity limit and an injection radius of 50 au. 

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M2n}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M2pv}
%   \caption{Position velocity diagram for model Model M2 for the CO J$=2\to1$. There is a low velocity component near the source that is originated from the outflow cavity and a high velocity component coming from the jet.}
%     \label{fig:M2}
% \end{figure}


\subsection{Jet velocity variability}

Then, in Model M3 we decided to use again an injection velocity of 200 km s$^{-1}$ keeping the injection radius at 50 au, but exploring the amplitude of the relative velocity variability, decreasing it from $8\%$ to $5\%$. This relative amplitude is offtently assumed and can be constrained through simulations. Even when the density map shows a similar structure to the previous models, that is, the length and the width are consistent with the observations, the PV diagram has a high velocity component that exhibits a steep gradient, suggesting that the jet itself is structured in velocity. Again, the intensity decreases along the jet. The mean velocity is also less than expected, but the structure, length, and width remain very similar to the observed ones.


\subsection{The jet acceleration}

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M3n}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/M3pv}
%     \caption{Position velocity diagram for model M3 for the CO J$=2\to1$. There is a low velocity component near the source that is originated from the outflow cavity and a high velocity component coming from the jet.}
%     \label{fig:M3}
% \end{figure}

Possibly the most intriguing feature showed by the Cep E PV diagram is that below 5$\times 10^3$ au, the CO emission accelerates with an exponential law from rest next to the source to the jet terminal velocity at larger distances. This is reproduced by the PV synthetic diagram for model M4 in Fig \ref{fig:M4}. In models M1 to M3, the PV diagram  clearly displays 2 components at low velocity ({\bf RANGE???}), corresponding to the cavity, and at high velocity, corresponding to the jet. 

In the case of Cep E, as in model M4, this behavior is explained as the interaction between the jet and material entraining it from the envelope. 
Interaction with the protostellar envelope ? \\ 


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/jetCO-CepE_r150-013.jpg}
%     \caption{Emissivity}
%     \label{fig:emissivity}
% \end{figure}


% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/pv-013-phi-40.eps}
%     \caption{PV Diagram}
%     \label{fig:pvd_sim}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/JetHH.jpeg}
%     \caption{Position velocity diagram for the Model D. The high and low velocity components are also noticeable as in Figure }
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/cavity_obs.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/cavity_sim.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/jet_obs.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/jet_sim.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


==> sec_observations.tex <==

\section{Observational constraints}

\subsection{The core}
\label{sec:obs}

CepE-mm is an intermediate-mass Class 0 protostellar core located in the Cepheus OB3 association at a distance of $819\pm 16\pc$  \citep{Karnath2019}, with a luminosity of $\approx 100\lsol$ \citep{Lefloch1996}. 

The dust emission spatial distribution was mapped by \cite{Lefloch1996} at a resolution of $11\arcsec$  with the 30m IRAM telescope. It revealed a relatively compact distribution centered on the infrared source IRAS23611+6142. %calculated the column density as $N(H_2)=$ $1.8\times10^{23}\cmmd$.
 We have adopted those physical conditions for the ambient gas in our numerical modelling (see Sect.~3.2).  

Based on continuum observations at $1.5\arcsec$ \cite{Ospina-Zamudio2018} recently showed that the source is actually a protostellar binary system with two components, A and B, distant by about $1.4\arcsec$, $\approx$ 1200au at the distance of the core, a result confirmed by observations of the NOEMA/SOLIS Large Program at $0.4\arcsec$ resolution (Lefloch et al. 2022 in prep). The most luminous component in the millimer continuum, Cep\,E-A, coincides with the nominal position of the IRAS source  IRAS23011+6126 at $\alpha(2000)=23^h03^m12^s.8$ and $\delta(2000)=61^\circ 42\arcmin26\arcsec$. Both protostars undergo episodes of active mass accretion as evidenced by the high-velocity outflows detected in the millimeter transitions of CO and SiO. 

\subsection{The outflow}
%Fig.1 
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/CO_specs.png}
    \caption{  
    CO $J$=2--1 emission detected towards CepE-mm with the PdBI at $1\arcsec$ resolution.
    {\em (left)} Velocity-integrated emission maps of observed in the CO $J$=2--1 in the different outflow components: a)outflow cavity walls (black), integrated between $-8$ and $-3$ km/s and $-14$ and $-19$ km/s in the northern and southern lobe, respectively; b) high-velocity jet between $-135$ and $-110$ km/s in the southern lobe (blue), and between $+40$ and $+80$ km/s in the northern lobe (red); c) terminal bowshock in magenta (green) in the north (south) between 84 and $97\kms$ ($-77$ and $-64\kms$). First contour and contour interval are $20\%$  and $10\%$ of the peak intensity of each component. Montage of spectra obtained at the offset positions marked in the pannels. Data are from \citet{Lefloch2015}. 
    }
    \label{fig:north}
\end{figure}

The emission of the molecular gas from the Cep\,E-mm protostellar outflow has been the subject of several observational studies \citep{Lefloch1996,Lefloch2015,Moro-Martin2001,Ospina-Zamudio2019}. 
\cite{Ospina-Zamudio2018} showed that Cep\,E-A is the protostar at the origin of the high-velocity outflow initially detected by \cite{Lefloch1996}. In what follows, we will refer to the high-velocity outflow/jet driven Cep\,E-A as "the outflow". 

%The source initially attracted attention because of the highly luminous mass-loss phenomena %generated in the near infrared, in particular in the \htwo\ rovibrational line S(1) v=1-0 at %$2.12\mu m$ \citep{Eisloeffel1996}, a probe of shocked molecular gas. At the same time, a high-velocity molecular outflow in emitting in the millimeter lines of CO and SiO \citep{Lefloch1996,LaddHodapp1997}, typical of young Class 0 protostars, was discovered towards the nominal position of the IRAS source.  Soon a second bipolar outflow with a position angle differing by $52\deg$ was reported by \cite{LaddHodapp1997}. 
CO
A first systematic study of the CO outflow in the $J$=2--1 line at $1\arcsec$ resolution with the IRAM interferometer was obtained by \cite{Lefloch2015}.
The molecular gas emission of each lobe, as mapped in the CO $J$=2--1 line, is displayed in Fig.~1. The emission can be divided into two different components: the low velocity cavity and the high velocity jet. The northern and southern jets propagate at different radial velocities of $+60\kms$ and $-125\kms$ (Fig.~1, right panel) and have a length of $25\arcsec$ and $21\arcsec$, respectively. If we take into account the Northern bowshock located at the apex of the northern cavity (see Fig.~1), the length of the northern lobe is actually $\approx 35\arcsec$, about 1.5 times longer than the southern lobe. 

Both lobes are terminated by a "bullet" in the North at offset position ($+7\arcsec$, $+36\arcsec$),  and in the south at offset position ($-9.3\arcsec$,$-22\arcsec$) with  Herbig-Haro object HH337 \citep{Ayala2000}.
The northern bullet was interpreted as the signature of the jet leaving the parental core \citep{Noriega-Crespo2014}.

The physical conditions (temperature, \htwo\ gas density) in the outflow/jet southern lobe were estimated by \citet{Lefloch2015} from a CO multi-rotational line study complemented  with CO $J$=2--1 observations at $1\arcsec$ angular resolution with the IRAM interferometer. 
The jet itself appears to consist mainly of warm (T=$80$--$100\K$), dense gas ($n(\htwo)$= (0.5--1.0)$\times 10^5\cmmt$. It appears rather massive, with a total mass of $0.02\msol$ and a diameter  of $\approx 1.7\arcsec$ (1500 au). The amount of momentum carried away by the jet ($\sim 1.7\msol\kms$) appears to be similar to that in the entrained ambient medium, and  supports the idea that the low velocity outflow is driven by the protostellar jet.  

The jet asymptotic radial velocities were measured on the CO 2--1 line profiles as  $+65\kms$ and $-125\kms$ in the northern and southern lobe, respectively (Fig.~1, right panel). The jet proper motions in both lobes were estimated by 
\cite{Noriega-Crespo2014} from combining multiple mid-infrared IRAC $4.5\mu m$ observations and \htwo\ $2.12 \mu m$ images at a difference of 16 years. {\bf We note that the revised distance of Cep\,E-mm (820 pc  instead of 730 pc previously) does not significantly affect the tangential velocities, which are now  $(70\pm 32)\kms$ and $(106\pm 29)\kms$ }
in the northern and southern lobes, respectively, nor the inclination angle of the jet with respect to the plane of the sky derived by \cite{Lefloch2015}, which is now $47\deg$ ($40\deg$ previously estimated) and the estimated dynamical age of the jet (about $10^3\yr$).  Cep\,E-mm is therefore one of the few protostellar jets for which a  full 3-D picture of the gas kinematics is available.




\subsection{Gas acceleration}



 Distribution of the CO emission as a function of velocity  along the main jet axis (see Position-Velocity diagram in Fig.~2) shows that the velocity is not constant at the resolution of the observations. The jet radial velocity increases gradually from ambient to its final value on a scale of $\approx 1\arcsec$. The radial velocity profile $V_r$ can be satisfyingly fitted by the relation 
 \begin{equation*}
 (V_r - V_{lsr})/V_0 = \exp(-z_0/z) 
 \end{equation*}
 where $V_0$ is the jet asymptotic radial velocity relative to the protostar in the northern ($+75\kms$) and southern ($-118\kms$) lobe, respectively. 
The length scale  $Z_0$ was determined from a best fitting procedure to the CO position-velocity diagram and found to be  equal to 693au and 590au in the northern and southern jet, respectively.
It is worth noticing that the independent fitting procedures on the northern and southern components yield a similar acceleration scales for the gas, of about $0.8\arcsec$ ($\sim 640$au). This length scale is marginally resolved by the present CO $J$=2--1 observations but is fully accessible to the SO 206176 MHz observations of the SOLIS project, at $\approx 0.4\arcsec$ resolution.  

\subsection{Periodic emission}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/knots.eps}
    \caption{Exponential fits for the intensity peaks extracted from the PV diagram for the nothern (red) and southern (blue) lobes of Cep E}
    \label{fig:fragments}
\end{figure}

The presence of CO knots, or "bullets", i.e. of structures of a few arcsec in diameter which display a higher emissivity in the jet was first reported by \citet{Lefloch2015}. They can be clearly seen  along both jet lobes in the CO $J$=2--1 emission map in Fig.~1. The fragmented structure is also apparent in the Position-Velocity diagram of the CO emission along the jet main axis (Fig.~2). We have reported the results of a systematic search for knots along the jet in Fig.~3, which displays the radial velocity of  knots as a function of distance to Cep\,E-A. 
%in CO J=2$\to$1 show a jet with a terminal constant velocity at large scales, but below %$5000$ au there is accelerated gas with a specific exponential law $v=v_{t}e^{-z/z_0}$, %where $v_t$is the terminal velocity and $z_0$ is a length scale. 
Such knots suggest the formation of internal working surfaces shocks propagating inside the jet with radial velocity fluctuations on the order of $\sim 10\kms$, hence of low amplitude with respect to the mean jet radial velocity. Interestingly,  search based on 
that are in correspondance in the norther and souther lobes with a periodicity: $\sim 130$
yr (Fig 2).

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/SO-PV.eps}
%     \caption{Position-Velocity diagram obtained from SO ($5_{4}$ to $4_{3}$) data through the main jet. First contour and contour interval are 10\% of the peak intensity.}
%     \label{fig:pvSO}
% \end{figure}






\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
          & North & South     \\
\hline
\hline
          &\multicolumn{2}{c|}{Cavity}    \\
\hline
Size  [$''$]      &       &     $22\times 10$      \\
\hline
$V_r$[km s$^{-1}$]   &       &    $-100;-11$        \\
\hline
\hline
&\multicolumn{2}{c|}{Jet}       \\
\hline
$V_t$  [km s$^{-1}$]   &   $62\pm29$    &  $94\pm26$        \\
\hline
$V_r$  [km s$^{-1}$]   &    $70$   &      $-116$     \\
\hline

Inclination $\phi$ [$^\circ$]    &       &    $40 $      \\
\hline
\hline
&\multicolumn{2}{c|}{HH377}     \\
\hline
$V_t$       &   -    &     $-90;-50$      \\
\hline
Size      &  -      &    4.5       \\
\hline
Position [$''$] &   -    &   26 \\
\hline
\end{tabular}
\caption{Cep E observed propierties}
\end{table}






